Real-time Neural-MPC: Deep Learning Model Predictive Control for Quadrotors and Agile Robotic Platforms

Model Predictive Control (MPC) has become a popular framework in embedded control for high-performance autonomous systems. However, to achieve good control performance using MPC, an accurate dynamics model is key. To maintain real-time operation, the dynamics models used on embedded systems have been limited to simple first-principle models, which substantially limits their representative power. In contrast to such simple models, machine learning approaches, specifically neural networks, have been shown to accurately model even complex dynamic effects, but their large computational complexity hindered combination with fast real-time iteration loops. With this work, we present Real-time Neural MPC, a framework to efficiently integrate large, complex neural network architectures as dynamics models within a model-predictive control pipeline. Our experiments, performed in simulation and the real world onboard a highly agile quadrotor platform, demonstrate the capabilities of the described system to run learned models with, previously infeasible, large modeling capacity using gradient-based online optimization MPC. Compared to prior implementations of neural networks in online optimization MPC we can leverage models of over 4000 times larger parametric capacity in a 50Hz real-time window on an embedded platform. Further, we show the feasibility of our framework on real-world problems by reducing the positional tracking error by up to 82% when compared to state-of-the-art MPC approaches without neural network dynamics.

==> resources/mse_simple_sim.tex <==
% This file was created with tikzplotlib v0.9.16.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}
\definecolor{color6}{rgb}{0.890196078431372,0.466666666666667,0.76078431372549}

\begin{groupplot}[group style={group size=3 by 1}]
\nextgroupplot[
tick align=outside,
tick pos=left,
title={RMSE [m] | Random},
x grid style={white!69.0196078431373!black},
xlabel={max vel [m/s]},
xmajorgrids,
xmin=6.76062575455423, xmax=12.6014541245677,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={RMSE [m]},
ymajorgrids,
ymin=-0.001, ymax=0.06,
ytick style={color=black}
]
\addplot [ultra thick, color0, dashed, mark=*, mark size=3, mark options={solid}]
table {%
7.0261179531912 0.00183028549162574
9.54516549680672 0.00618157476866314
10.5358525783262 0.00896270669394923
11.2417887251059 0.0115678223079637
12.3359619259307 0.0165299150369151
};
\addplot [semithick, color1, dashed, mark=*, mark size=3, mark options={solid}]
table {%
7.0261179531912 0.12219826577615
9.54516549680672 0.153094134175285
10.5358525783262 0.162168196737711
11.2417887251059 0.167770488283221
12.3359619259307 0.17906806047338
};
\addplot [semithick, color2, dashed, mark=*, mark size=3, mark options={solid}]
table {%
7.0261179531912 0.0548756582971127
9.54516549680672 0.0557707722258428
10.5358525783262 0.054267651303231
11.2417887251059 0.052839680589732
12.3359619259307 0.0511944558061592
};
\addplot [semithick, color3, dashed, mark=*, mark size=3, mark options={solid}]
table {%
7.0261179531912 0.0204051616490007
9.54516549680672 0.0268786576004875
10.5358525783262 0.0295303362363602
11.2417887251059 0.0312854011199185
12.3359619259307 0.0341864389689094
};
\addplot [semithick, color4, dashed, mark=*, mark size=3, mark options={solid}]
table {%
7.0261179531912 0.0334167874110753
9.54516549680672 0.0357709874256417
10.5358525783262 0.0361958908424773
11.2417887251059 0.0361569202302672
12.3359619259307 0.0369035476541776
};
\addplot [semithick, color5, dashed, mark=*, mark size=3, mark options={solid}]
table {%
7.0261179531912 0.0212032030093479
9.54516549680672 0.027042273882087
10.5358525783262 0.0298900701498069
11.2417887251059 0.0318434073176609
12.3359619259307 0.0350955166885494
};
\addplot [semithick, color6, dashed, mark=*, mark size=3, mark options={solid}]
table {%
7.0261179531912 0.0176639638653371
9.54516549680672 0.0244629226545807
10.5358525783262 0.0270557617481065
11.2417887251059 0.028812785007971
12.3359619259307 0.0315431289809773
};
\addplot [semithick, white!49.8039215686275!black, dashed, mark=*, mark size=3, mark options={solid}]
table {%
7.0261179531912 0.0175491391626581
9.54516549680672 0.024258892715482
10.5358525783262 0.0269102099720437
11.2417887251059 0.0286951843901753
12.3359619259307 0.0315816541753861
};

\nextgroupplot[
tick align=outside,
tick pos=left,
title={RMSE [m] | Circle},
x grid style={white!69.0196078431373!black},
xlabel={max vel [m/s]},
xmajorgrids,
xmin=1.60245501175827, xmax=13.3537917646522,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ymajorgrids,
ymin=-0.001, ymax=0.06,
ytick style={color=black}
]
\addplot [ultra thick, color0, dashed, mark=*, mark size=3, mark options={solid}]
table {%
2.13660668234436 0.000419589471891745
4.80736503527482 0.00017964591490403
7.47812338820527 0.00050172215494334
10.1488817411357 0.0010639777470892
12.8196400940662 0.00189533829425466
};
\addplot [semithick, color1, dashed, mark=*, mark size=3, mark options={solid}]
table {%
2.13660668234436 0.0494734064278136
4.80736503527482 0.134176073110979
7.47812338820527 0.213029790050188
10.1488817411357 0.27690786487746
12.8196400940662 0.333598036894481
};
\addplot [semithick, color2, dashed, mark=*, mark size=3, mark options={solid}]
table {%
2.13660668234436 0.042896118054657
4.80736503527482 0.0499692547329007
7.47812338820527 0.046819100789533
10.1488817411357 0.0458829020964005
12.8196400940662 0.0425755133835506
};
\addplot [semithick, color3, dashed, mark=*, mark size=3, mark options={solid}]
table {%
2.13660668234436 0.0128816195055173
4.80736503527482 0.017297648607279
7.47812338820527 0.0228956797896126
10.1488817411357 0.0277114787182369
12.8196400940662 0.0293994969536733
};
\addplot [semithick, color4, dashed, mark=*, mark size=3, mark options={solid}]
table {%
2.13660668234436 0.026504494682952
4.80736503527482 0.0310349205551213
7.47812338820527 0.0299823300621795
10.1488817411357 0.0306778393765262
12.8196400940662 0.0302792217004344
};
\addplot [semithick, color5, dashed, mark=*, mark size=3, mark options={solid}]
table {%
2.13660668234436 0.0159520533013479
4.80736503527482 0.0220497693947658
7.47812338820527 0.0246305716014441
10.1488817411357 0.027568718861843
12.8196400940662 0.0279006022294454
};
\addplot [semithick, color6, dashed, mark=*, mark size=3, mark options={solid}]
table {%
2.13660668234436 0.0114764070391561
4.80736503527482 0.0149587703431082
7.47812338820527 0.0205386459400568
10.1488817411357 0.0256611275650241
12.8196400940662 0.0249107141620845
};
\addplot [semithick, white!49.8039215686275!black, dashed, mark=*, mark size=3, mark options={solid}]
table {%
2.13660668234436 0.011404572448894
4.80736503527482 0.0148288998864887
7.47812338820527 0.0206681107372962
10.1488817411357 0.0253682450245887
12.8196400940662 0.0246610043724947
};

\nextgroupplot[
tick align=outside,
tick pos=left,
title={RMSE [m] | Lemniscate},
x grid style={white!69.0196078431373!black},
xlabel={max vel [m/s]},
xmajorgrids,
xmin=2.13492967215171, xmax=18.8250637073041,
xtick style={color=black},
xtick={2,4,6,8,10,12,14,16,18,20},
xticklabels={0.0,2.5,5.0,7.5,10.0,12.5,15.0,17.5,20.0,},
y grid style={white!69.0196078431373!black},
ymajorgrids,
ymin=-0.001, ymax=0.06,
ytick style={color=black}
]
\addplot [ultra thick, color0, dashed, mark=*, mark size=3, mark options={solid}]
table {%
2.893572128295 7.22563593609974e-05
5.9172632332243 0.000727762657291357
10.500403772372 0.00318439081298801
13.9597424215952 0.0109385046395464
18.0664212511608 0.0280126286380616
};
\addplot [semithick, color1, dashed, mark=*, mark size=3, mark options={solid}]
table {%
2.893572128295 0.0499872813658149
5.9172632332243 0.123957135477562
10.500403772372 0.186886656331651
13.9597424215952 0.243811018359795
18.0664212511608 0.296565238486624
};
\addplot [semithick, color2, dashed, mark=*, mark size=3, mark options={solid}]
table {%
2.893572128295 0.0446671750434128
5.9172632332243 0.0481034485522777
10.500403772372 0.0523769888657313
13.9597424215952 0.0424641669393065
18.0664212511608 0.0587467578141734
};
\addplot [semithick, color3, dashed, mark=*, mark size=3, mark options={solid}]
table {%
2.893572128295 0.0151534756167745
5.9172632332243 0.0184117189926839
10.500403772372 0.0250251959525734
13.9597424215952 0.027396494957712
18.0664212511608 0.0433649510164499
};
\addplot [semithick, color4, dashed, mark=*, mark size=3, mark options={solid}]
table {%
2.893572128295 0.0268617385481395
5.9172632332243 0.0297052021494501
10.500403772372 0.0318890932879892
13.9597424215952 0.0308532763022243
18.0664212511608 0.0477400610414831
};
\addplot [semithick, color5, dashed, mark=*, mark size=3, mark options={solid}]
table {%
2.893572128295 0.0164544384735954
5.9172632332243 0.0214329868836112
10.500403772372 0.0257270924953106
13.9597424215952 0.0276374907742935
18.0664212511608 0.0429907163150912
};
\addplot [semithick, color6, dashed, mark=*, mark size=3, mark options={solid}]
table {%
2.893572128295 0.013201573710542
5.9172632332243 0.0168683162888948
10.500403772372 0.0222531371394148
13.9597424215952 0.0264143362330949
18.0664212511608 0.042399709033078
};
\addplot [semithick, white!49.8039215686275!black, dashed, mark=*, mark size=3, mark options={solid}]
table {%
2.893572128295 0.0132037898544637
5.9172632332243 0.0168320802407788
10.500403772372 0.0219638114679166
13.9597424215952 0.026123220143767
18.0664212511608 0.0429060667393653
};
\end{groupplot}

\end{tikzpicture}


==> resources/t_opt_simple_sim.tex <==
% This file was created with tikzplotlib v0.9.16.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}

\begin{axis}[
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Max vel [m/s]},
xmin=1.34011595390353, xmax=18.8629119796017,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Mean MPC loop time (s)},
ymin=0.000413987638219296, ymax=0.00814168370272113,
ytick style={color=black}
]
\addplot [semithick, color0]
table {%
2.13660668234436 0.000768659909566243
2.893572128295 0.000823696454366048
7.0261179531912 0.000796505409323012
12.3359619259307 0.000789686795827505
12.8196400940662 0.000765246550242106
18.0664212511608 0.000777919292449951
};
\addplot [semithick, color1]
table {%
2.13660668234436 0.000769658486048381
2.893572128295 0.00078135093053182
7.0261179531912 0.000773275945513568
12.3359619259307 0.000785167152817185
12.8196400940662 0.000771373510360718
18.0664212511608 0.000781519015630086
};
\addplot [semithick, color2]
table {%
2.13660668234436 0.00280134638150533
2.893572128295 0.0027118456363678
7.0261179531912 0.00289647274281835
12.3359619259307 0.00309301969167349
12.8196400940662 0.0027208944161733
18.0664212511608 0.0027451233069102
};
\addplot [semithick, color3]
table {%
2.13660668234436 0.00460212548573812
2.893572128295 0.0044547172387441
7.0261179531912 0.0043636092052254
12.3359619259307 0.00439584512968321
12.8196400940662 0.00450701117515564
18.0664212511608 0.00449432651201884
};
\addplot [semithick, color4]
table {%
2.13660668234436 0.00761676907539368
2.893572128295 0.00759796063105265
7.0261179531912 0.00779042479069832
12.3359619259307 0.00762136304700697
12.8196400940662 0.00769907474517822
18.0664212511608 0.0076045020421346
};
\addplot [semithick, color5]
table {%
2.13660668234436 0.0020306666692098
2.893572128295 0.0025309693813324
7.0261179531912 0.00209133136437744
12.3359619259307 0.00204941388723013
12.8196400940662 0.00223254799842834
18.0664212511608 0.00234382669130961
};
\end{axis}

\end{tikzpicture}

